TADOC: Text Analytics Directly on Compression

This article provides a comprehensive description of Text Analytics Directly on Compression (TADOC), which enables direct document analytics on compressed textual data. The article explains the concept of TADOC and the challenges to its effective realizations. Additionally, a series of guidelines and technical solutions that effectively address those challenges, including the adoption of a hierarchical compression method and a set of novel algorithms and data structure designs, are presented. Experiments on six data analytics tasks of various complexities show that TADOC can save 90.8% storage space and 87.9% memory usage, while halving data processing times.

==> insert_7.tex <==

\subsubsection{
\cred{Word Co-Occurrence}
}


In the evaluation,
we compare the co-occurrence using TADOC with the compressed datasets \texttt{D} and \texttt{E},
and the original co-occurrence with the related uncompressed datasets.
We use default parameters in the comparison.
Experiment shows that TADOC saves 35.5\% time on average in execution;
%Experiment shows that the {\em compression-based direct processing} saves \cred{XXX}\% time on average in the pre-processing stage of the matrix construction;
the original implementation needs 33.3 seconds for dataset \texttt{D} and 42.4 seconds for dataset \texttt{E},
while ours using \texttt{CD} only needs 25.0 (\texttt{D}) and 22.8 (\texttt{E}) seconds.
The performance benefit mainly comes from the data reuse in TADOC.

\subsubsection{\cred{TFIDF}}

In the evaluation,
we test the TFIDF using dataset \texttt{D} and \texttt{E}.
The baseline version needs 16.0 seconds for processing dataset \texttt{D},
%The baseline version needs 16.0 seconds for processing dataset \texttt{D},
and 18.9 seconds for \texttt{E}.
%and 19.5 seconds for \texttt{E}.
When using \texttt{CD},
we only need 9.9 seconds for dataset \texttt{D},
and 8.4 seconds for \texttt{E},
which implies that
TADOC brings about 46.3\% performance benefits.




\subsubsection{
\cred{Word2vec}
}

We conduct experiments on dataset \texttt{D} and \texttt{E}.
The original preprocessing time are 29.1 (\texttt{D}) and 37.4 (\texttt{E}) seconds,
while the preprocessing time with \texttt{CD} are 7.0 (\texttt{D}) and 7.1 (\texttt{E}) seconds.
Experiments show that TADOC saves 78.7\% preprocessing time.
The training time of word2vec is much longer than the processing time (2085.1 seconds for \texttt{D} and 2895.2 seconds for \texttt{E}).
Although the time savings are small compared to the long training time,
the word2vec can still enjoy the space benefit since it can directly read the input from the compressed data.



\subsubsection{\cred{LDA}}
We compare the LDA using \texttt{CD} with the baseline on the single node server with dataset \texttt{D} and \texttt{E}.
In the first stage, for dataset \texttt{D}, the time of LDA using \texttt{CD} and without using \texttt{CD} are 20.3 and 45.8 seconds separately,
while for dataset \texttt{E}, the time using and without using \texttt{CD} are 14.9 and 67.4 seconds,
which indicates that TADOC saves 66\% preprocessing time on average.
We further analyze the IO time and computation time in this stage,
and experiment shows that \texttt{CD} saves 88.0\% IO time and 61.7\% computation time.
The second stage takes 426 (\texttt{D}) and 485 (\texttt{E}) seconds for both baseline and \texttt{CD},
because they process the same data.
With training process involved,
the time benefit is not that much.
However, we can still enjoy the large space benefits from the compressed format of \texttt{CD}.



